Thermal Safety and Real-Time Predictability on Heterogeneous Embedded SoC Platforms

Recent embedded systems are designed with high-performance System-on-Chips (SoCs) to satisfy the computational needs of complex applications widely used in real life, such as airplane controllers, autonomous driving automobiles, medical devices, drones, and hand-held devices. Modern SoCs integrate multi-core CPUs and various types of accelerators including GPUs and DSPs. Uncontrolled heat dissipation is one of the main sources of interference that can adversely affect the reliability and real-time performance of safety-critical applications. The mechanisms currently available to protect SoCs from overheating, such as frequency throttling or core shutdown, may exacerbate the problem as they cause unpredictable delay and deadline misses. Dynamic changes in ambient temperature further increase the difficulty of solving this problem. This dissertation addresses the challenges caused by thermal interference in real-time mixed-criticality systems built with heterogeneous embedded SoC platforms. We propose a novel thermal-aware system framework with analytical timing and thermal models to guarantee safe execution of real-time tasks under the thermal constraints of a multi-core CPU/GPU integrated SoC. For mixed-criticality tasks, the proposed framework bounds the heat generation of the system at each criticality level and provides different levels of assurance against ambient temperature changes. In addition, we propose a data-driven thermal parameter estimation scheme that is directly applicable to MCSs built with commercial-off-the-shelf multi-core processors to obtain a precise thermal model without using special measurement instruments or access to proprietary information. The practicality and effectiveness of our solutions have been evaluated using real SoC platforms and our contributions will help develop systems with thermal safety and real-time predictability.

==> Chapter4/6-floorplan/0-floorplan.tex <==

 

==> Chapter4/8-Evaluation/7_case_study.tex <==
\subsection{Case study on intel processor}

==> Chapter4/prelim.tex <==

\section{\new{Background on Thermal Behavior}}
\label{sec:background}
\new{ALI::: change  here ALSO}
In this section, we briefly introduce the thermal model used in this paper. It depends on power consumption, heat dissipation, and convective heat transfer between adjacent power-consuming resource components, which includes CPU cores, CPU peripherals, GPU, caches, and other IPs.

\smallskip\noindent\textbf{Power model.} The total power consumption of CMOS circuits is modeled as the summation of dynamic and static powers ($P(t) = P_D(t) + P_S(t)$)\cite{4484694}. Static power $P_S$ depends on the semiconductor technology and the operating temperature caused by current leakage. Therefore, static power presents when a power resource is switched on. Static power can be modeled as a linear function of temperature. Hence, static power is $P_S(t) = k_1 \theta(t) + k_2 $, where $k_1$ and $k_2$ are technology-dependent system constants, and $\theta$ is the operating temperature \cite{4212027}. Dynamic power $P_D(t)$ is the amount of power consumption due to the processor operating frequency $f$, modeled as $P_D = k_0 f^s$, where $f$ and $k_0$ are system constants that depend on the semiconductor technology. It is worth noting that in this paper, our framework runs processor cores at fixed operating frequency to obtain predictable worst-case task execution time. Consequently, the total power is the function of $\theta(t)$ because the other factors such as frequency remain invariant during execution. 


\smallskip\noindent\textbf{Uni-processor thermal model.} With respect to the power function\cite{4212027, 4484694}, the thermal model of a uni-processor is modeled as an RC circuit in the literature \cite{4484694, 6200041, Skadron}. According to the Fourier's Law \cite{wang2010schedulability}, the temperature of a core $\theta(t)$ at time $t$ can be derived by solving the following differential equation\footnote{Details are available in~\cite{DSouza2017ThermalIO} and \cite{Ahmed2017}.}:
\begin{equation}
     \theta(t) = \alpha + (\theta(t_0)-\alpha) e^{\beta t}
     \label{eq:tempActive}
\end{equation}
where $\alpha > 0$ and $\beta < 0 $ are constants. 

Most operating systems in embedding platforms transition the processor to the sleep state when there is no task execution. Therefore, the power consumption can be assumed to be negligible in such a case. The thermal function in the sleep state (\textit{aka} cooling phase) where the frequency is switched off can be modeled as:
\begin{equation}
    \theta(t) = \theta(t_0) e^{\beta t}.
    \label{eq:tempCool}
\end{equation}
 because in the cooling phase, $a = 0$.
 
\smallskip\noindent\textbf{Homogeneous multi-core thermal model.} With the presence of multiple cores and other power-consuming resources, there is heat dissipation not only to ambient but also between nodes. In this paper, we only consider CPU cores as power-consuming nodes because other IPs consume much less power than them, thereby causing negligible thermal effects. 

In such a multi-core system with thermal transition between processing cores, the temperature of a core depends not only on its current temperature and power consumption, but also on those of adjacent cores.  Prior work~\cite{6629322} showed that the temperature of each core at time $t+\Delta$ can be modeled with acceptable accuracy as follows:
\[ \Theta(t+\Delta) = A \times P(t+\Delta) + \Gamma \times \Theta(t)  \]
where $A$ is  $m \times m$ matrix, and $\Gamma$, $P$ and $\Theta$ are $m \times 1$ matrices, respectively. One can interpret the thermal model as a function of the current temperature and heat produced by execution and convection between cores. 
Hence, according to the thermal composability characteristics of heat transfer~\cite{Ahmed2017} with the initial temperature of $\theta(t_0)$, the temperature after $t$ time units is given by:
\begin{equation}
\theta_i(t_0+t) = \alpha + (\theta(t_0)-\alpha) e^{\beta t} +  \sum_{j=1}^{m} \gamma_{ij} \theta_j(t_0+t).
    \label{eq:tempCompo}
\end{equation} 
